Enhancing Privacy in Federated Learning: Secure Aggregation for Real-World Healthcare Applications

Deploying federated learning (FL) in real-world scenarios, particularly in healthcare, poses challenges in communication and security. In particular, with respect to the federated aggregation procedure, researchers have been focusing on the study of secure aggregation (SA) schemes to provide privacy guarantees over the model's parameters transmitted by the clients. Nevertheless, the practical availability of SA in currently available FL frameworks is currently limited, due to computational and communication bottlenecks. To fill this gap, this study explores the implementation of SA within the open-source Fed-BioMed framework. We implement and compare two SA protocols, Joye-Libert (JL) and Low Overhead Masking (LOM), by providing extensive benchmarks in a panel of healthcare data analysis problems. Our theoretical and experimental evaluations on four datasets demonstrate that SA protocols effectively protect privacy while maintaining task accuracy. Computational overhead during training is less than 1% on a CPU and less than 50% on a GPU for large models, with protection phases taking less than 10 seconds. Incorporating SA into Fed-BioMed impacts task accuracy by no more than 2% compared to non-SA scenarios. Overall this study demonstrates the feasibility of SA in real-world healthcare applications and contributes in reducing the gap towards the adoption of privacy-preserving technologies in sensitive applications.

==> latex_files/buildingblocks.tex <==
In this Section we explain the cryptographics primitives used to implement SA in Fed-BioMed.
\paragraph{Key Agreement Scheme.} Diffie-Hellman key agreement scheme (KA) is parametrized with a security parameter $\lambda$ consisting of three PPT (Probabilistic Polynomial Time) algorithms:

$\bullet$  $pp \gets \textbf{KA.Param}(\lambda)$: Given a security parameter $\lambda$, it generates two large primes $p$ and $q$ such that $q$ divides $p - 1$ and outputs an element $g \in \mathbb{Z}^*_p$ of order $q$, $p=(g,p,q)$.
    
$\bullet$ $(c^{PK}_u, c^{SK}_u) \gets \textbf{KA.Gen}(pp)$:  generates key pairs from the public parameters where $(c^{PK}_u, c^{SK}_u) = (g^a, a)$ and $a$ is chosen uniformly at random from $\mathbb{Z}^*_q$.
    
$\bullet$ $c_{u,v} \gets \textbf{KA.Agree}(pp, c^{SK}_u, c^{PK}_v, H)$: uses the private key of user $u$, the public key of user $v$, and  generate a share secret  as $c_{u,v} = (c^{PK}_v)^{c^{SK}_u}$.

\paragraph{Shamir Secret Sharing.} A $t$-out-of-$n$ Shamir Secret Sharing scheme \cite{shamir79}, denoted as SS, defined in a field $\mathbb{F}_p$, where $p$ is a prime number, consists of two PPT algorithms:

    $\bullet$ $\{(u,[s]_u)\}_{u \in \users} \gets $\textbf{SS.Share}$(s,t,\users)$: it splits a secret $s \in \mathbb{F}_p$ into $n$ shares $[s]_u \in \mathbb{F}_p$, each of them for one client $u \in \users$.
    Let $t$ be the reconstruction threshold
     The algorithm first generates a polynomial $p(x)$ of uniformly random coefficients and degree $t-1$ such as $p(0) = s$. It then computes $p(u) = [s]_u $ for all $u \in \users$. 
     
    $\bullet$ $s \gets $\textbf{SS.Recon}$(\{(u,[s]_u)\}_{u \in \users'},t)$: it reconstructs the secret $s \in \mathbb{F}_p$ using at least $t$ shares. It is required that $\users' \subseteq \users$ and $|\users'| \geq t$. It uses the Lagrange interpolation to compute the value $p(0)=s$ as follows (all operation are in the field $\mathbb{F}_p$):
    $$ s = \sum\limits_{ u \in \users'}\lambda_u [s]_u \qquad \textnormal{where} \qquad  \lambda_u = \prod\limits_{u \in \users' \setminus \{u\}}{\frac{v}{v-u}}$$


\paragraph{Joye Libert.}
The \tbf{Joye Libert (JL)} scheme \cite{JL2013} is defined with three algorithms.

    
$\bullet$  $(sk_0, \{sk_u\}_{u \in \users}, pp) \gets \tbf{JL.Setup}(\lambda)$: Given the security parameter $\lambda$, it generates two large, equal-size prime numbers $p$ and $q$ and sets the modulus $N = pq$.  It randomly generates $n$ clients secret keys $sk_u \in \mathbb{Z}_{N^2}$ and computes the aggregator secret key $sk_0 = -\sum_{u=1}^n{sk_u}$. Then, it defines a cryptographic hash function $F : \mathbb{Z} \rightarrow \znnm$.  It outputs the $n+1$ secret keys and the public parameters $pp^{JL}=(N,F)$.

$\bullet$  $\sencsync \gets \tbf{JL.Protect}(pp,sk_u,\tau,\sinputsync)$: This algorithm encrypts private input $\sinputsync \in \mathbb{Z}_N$ for time period $\tau$ using secret key $sk_u \in \znn$, resulting in ciphertext $\sencsync= (1+\sinputsync N)\cdot F(\tau)^{sk_u} \mod N^2$. 

$\bullet$  $\saggsync \gets \tbf{JL.Agg}(pp, sk_0,\tau, \{\sencsync\}_{\uuu})$: This algorithm aggregates the $n$ protected inputs from clients received at time period $\tau$ to obtain $y_{\tau} = \prod_{u=1}^n{\sencsync} $.
It then decrypts $y_{\tau}$ to recover the plaintext aggregate $\saggsync = \sum_{u=1}^n{\sinputsync}= (F(\tau)^{-sk_0} \cdot y_{\tau}-1)/N \mod N$.
For security details please refer to \cite{JL2013}.
\paragraph{Low-Overhead Masking.} The \textbf{Low-Overhead Masking(LOM)} \cite{kursawe2011privacy} scheme is defined with three algorithms.
    
$\bullet$  $(\{s_{u,v}\}_{u \in \users}, pp) \gets \textbf{LOM.Setup}(\lambda)$: Given the security parameter \(\lambda\), this algorithm initializes a pseudorandom function \(G\) and a domain $M$. It generates shared keys between each pair of clients \(s_{u,v} \). It outputs the user secret keys \(\{s_{u,v}\}_{u,v \in \users}\) and the public parameters \(pp = (G, D)\).

$\bullet$  $\sencsync \gets \textbf{LOM.Protect}(pp,\{s_{u,v}\}_{\forall v \in \users \setminus {u}}, \tau, \sinputsync)$: This algorithm encrypts the private input \(\sinputsync \in \mathbb{Z}_D\) for time period \(\tau\) secret key \(b_{u, \tau} =\sum_{v \neq u}^n (-1)^{u<v} G(s_{u,v} \| \tau)\) and encrypts the input as \(\sencsync = (\sinputsync + b_{u, \tau}) \mod D\).

$\bullet$  $\saggsync \gets \textbf{LOM.Aggregate}(pp,\{\sencsync\}_{u \in \users})$: This algorithm aggregates the \(n\) protected inputs from clients received at time period \(\tau\) to obtain recover the plaintext aggregate \(\saggsync = \sum_{u=1}^n{\sencsync} \).
For security details please refer to \cite{kursawe2011privacy}.

==> protocols/protocol_v2.tex <==
% \begin{figure*}[t]
% \centering
% \raggedright
  
%   \textbf{Parties:} Researcher, Nodes ~$\users
% $ and selected Nodes $\selected$, s.t $|\users| = n_{tot}$ and $\selected =n$.
% \raggedright
  
%   \smallskip
%   \scalebox{0.8}{
%   \begin{minipage}[t]{.65\textwidth}
%             \textbf{Public Parameters:}  $(\perp, pp^{LOM}) \gets \textbf{LOM.Setup}(\lambda)$           
%             \raggedright
%             \textbf{Setup - Key Registration:} 
%                 \begin{description}
%                 \item{Node $u \in \users$:}
%                     \begin{enumerate}
%                 \item  $c_u^{SK}, c_u^{PK} \gets \tbf{KA.Gen}(pp^{KA})$ 
%                 \item Send $c_u^{PK}$ to Researcher
%             \end{enumerate}
%             %                 \item{Node $u \in \users$:}
%             %         \begin{enumerate}
%             %     \item  $c_u^{SK}, c_u^{PK} \gets \tbf{KA.Gen}(pp^{KA})$             
%             % \end{enumerate}
%                 \end{description}

%               \textbf{Setup - Key Setup:}
%                               \begin{description}
%                 \item{Reseacher:}
%                     \begin{enumerate}
%                 \item  Collect $\{c_u^{PK}\}_{\uuu}$  and send to nodes $\users$.
%             \end{enumerate}
%             \end{description}
%                 \begin{description}
%                 \item{Node $u \in \users$:}
%                     \begin{enumerate}
%                 \item  $\forall v \in \users \setminus\{u\}$,  $s_{u,v} \gets \tbf{KA.agree}(pp^{KA}, c_u^{SK}, c_v^{PK})$             
%             \end{enumerate}


%                 \end{description}
%               \end{minipage}
  
% \begin{minipage}[t]{.65\textwidth}
%               \textbf{Online - Protection (round $\tau$, selected Nodes $\selected$):} 
% \begin{description}
%     \item{Node $u \in \selected$: \textcolor{gray}{\textit{ // Protect private input}}}
%         \begin{enumerate}
%             \item  $ \vencsync \gets \tbf{LOM.Protect}(pp^{LOM}, \{s_{u,v}\}_{\forall v \in \selected \setminus {u}}, \tau, \vinputsync)$
%             \item Send $\vencsync$ to \textit{Researcher}.
%             \end{enumerate}
%                 \item{Researcher:
%                \textcolor{gray}{\textit{// Complete the aggregation}}}
%                 \begin{enumerate}
%                     \item Collect $\{\vencsync\}_{\forall u \in \selected}$.
%                     \item $\vagg \gets \tbf{LOM.Agg}(pp^{LOM}, \{\vencsync\}_{\forall u \in \selected}) $
%                 \end{enumerate}   
%                 \end{description}
% \end{minipage}
%             }
% 	\caption{LOM protocol implemented in Fed-BioMed}
%             \label{fig:protocol_v2}
%     \end{figure*}

